Hardness results for Multimarginal Optimal Transport problems

Multimarginal Optimal Transport (MOT) is the problem of linear programming over joint probability distributions with fixed marginals. A key issue in many applications is the complexity of solving MOT: the linear program has exponential size in the number of marginals k and their support sizes n. A recent line of work has shown that MOT is poly(n,k)-time solvable for certain families of costs that have poly(n,k)-size implicit representations. However, it is unclear what further families of costs this line of algorithmic research can encompass. In order to understand these fundamental limitations, this paper initiates the study of intractability results for MOT. Our main technical contribution is developing a toolkit for proving NP-hardness and inapproximability results for MOT problems. We demonstrate this toolkit by using it to establish the intractability of a number of MOT problems studied in the literature that have resisted previous algorithmic efforts. For instance, we provide evidence that repulsive costs make MOT intractable by showing that several such problems of interest are NP-hard to solve--even approximately.

==> sections/app_partial.tex <==
\section{Extension to partial marginal constraints}\label{app:partial}

Here we briefly remark that our algorithmic results extend to the setting where only a subset $\cI \subseteq [k]$ of the marginals are constrained. We denote this generalization to partial marginal constraints by $\MOT'$. Given $\cI \subseteq [k]$, and measures $\{\mu_i\}_{i \in \cI} \subset \Delta_n$, the partially-fixed transportation polytope is
$$\cM_{\cI}(\{\mu_i\}_{i \in \cI}) := \{P \in \Rpntk : m_i(P) = \mu_i, \; \forall i \in \cI\}.$$ For cost $C \in \Rntk$, measures $\{\mu_i\}_{i \in \cI} \subset \Delta_n$, and regularization $\eta > 0$, we define the $\MOT'$ and $\RMOT'$ problems with partially-fixed marginals as follows.
\begin{align}
\min_{P \in \cM_{\cI}(\{\mu_i\}_{i \in \cI})} \langle P, C \rangle. \label{MOTprime} \tag{MOT'}
\end{align}
\begin{align}
	\min_{P \in \cM_{\cI}(\{\mu_i\}_{i \in \cI})} \langle P, C \rangle - \eta^{-1} H(P).
	\label{RMOTprime}
	\tag{RMOT'}
\end{align}
In analogy with the fixed-marginal case, the $\MinO$, $\AMinO$, and $\SMinO$ oracles are sufficient to solve $\MOT'$ in polynomial time:
\begin{theorem}[Algorithmic results extend to partially-fixed marginals] \label{thm:apppartial}
Theorem~\ref{thm:ellipmotp} ($\ELLIP$), Theorem~\ref{thm:mwumotp} ($\MWU$), and Theorems~\ref{thm:sink-rmot} and~\ref{thm:sink-mot} $(\Sink)$ hold if we replace \eqref{MOT} by \eqref{MOTprime} and \eqref{RMOT} by \eqref{RMOTprime}. 
\end{theorem}

The proofs of these modified theorems are nearly identical and thus omitted. As in the fully-fixed marginals case, the core intuition is that access to $\MinO$ is sufficient to implement a separating hyperplane oracle for the dual $\MOT'$ problem
\begin{align}
& \max_{(p_i)_{i \in \cI} \in (\Rn)^{\cI}} \sum_{i \in \cI} \langle p_i, \mu_i \rangle \tag{MOT-D'}
\quad \text{subject to} \quad  
C_{j_1,\dots,j_k} - \sum_{i \in \cI} [p_i]_{j_i} \geq 0, \; \forall (j_1,\dots,j_k) \in [n]^k.
\label{MOT-Dprime} 
\end{align}



==> sections/appx_dft_hard.tex <==
\section{Proof of Proposition~\ref{prop:hard-dft-approx}}

By Theorem~\ref{thm:main:approx}, it suffices to prove that approximating $\MinO_C(0)$ up to $\leq 1/\poly(n,k)$ additive error is $\NP$-hard.

We modify the proof of \citep[Theorem 5]{adamson2020hardness} to prove hardness of $1/\poly(n,k)$-additive approximation of \eqref{eq:modifieddftobjective}. Note that for the parameters $A_{\pm}, B_{\pm}, C_{\pm}$ chosen in Lemma 1 of \citep[Theorem 5]{adamson2020hardness}, inequalities (1)-(3) of \citep{adamson2020hardness} are met strictly, with a small polynomial gap of at least $1/n^{10}$: i.e., for large enough $n$,
\begin{align*}
	&\frac{A_+}{e^{B_+ n}} - \frac{C_+}{n^6} + \frac{1}{n} + \frac{A_-}{e^{B- \sqrt{1+n^2}}} - \frac{C_-}{(1+n^2)^3} - \frac{1}{\sqrt{1+n^2}} \geq |\frac{A_-}{e^{B_-}} - C_- - 1| + 1/n^{10} \\
	&n^2 |\frac{A_+}{e^{B_+ r}} - \frac{C_+}{r^6} + \frac{1}{r} + \frac{A_-}{e^{B- \sqrt{1+r^2}}} - \frac{C_-}{(1+r^2)^3} - \frac{1}{\sqrt{1+r^2}}| \leq |\frac{A_-}{e^{B_-}} - C_- - 1| - 1/n^{10}, & r \geq \sqrt{2n} \\
	& \frac{A_+}{e^{B_+ r}} - \frac{C_+}{r^6} + \frac{1}{r} + \frac{A_-}{e^{B- \sqrt{1+r^2}}} - \frac{C_-}{(1+r^2)^3} - \frac{1}{\sqrt{1+r^2}} > 1/n^{10}, & r \geq \sqrt{2n}.
\end{align*}
Tracing through the reasoning of Lemmas 2, 3, and 4 of \citep{adamson2020hardness}, this gap implies that a $\pm 0.49/n^{10}$ approximation to the objective~\eqref{eq:modifieddftobjective} suffices to determine whether or not the construction in \citep[Theorem 5]{adamson2020hardness} encodes a graph with an independent set of size $k/2$. This proves NP-hardness of $\pm 0.49/n^{10}$ approximation for~\eqref{eq:modifieddftobjective}. 
